Boosting Weakly-Supervised Image Segmentation via Representation, Transform, and Compensator

Weakly-supervised image segmentation (WSIS) is a critical task in computer vision that relies on image-level class labels. Multi-stage training procedures have been widely used in existing WSIS approaches to obtain high-quality pseudo-masks as ground-truth, resulting in significant progress. However, single-stage WSIS methods have recently gained attention due to their potential for simplifying training procedures, despite often suffering from low-quality pseudo-masks that limit their practical applications. To address this issue, we propose a novel single-stage WSIS method that utilizes a siamese network with contrastive learning to improve the quality of class activation maps (CAMs) and achieve a self-refinement process. Our approach employs a cross-representation refinement method that expands reliable object regions by utilizing different feature representations from the backbone. Additionally, we introduce a cross-transform regularization module that learns robust class prototypes for contrastive learning and captures global context information to feed back rough CAMs, thereby improving the quality of CAMs. Our final high-quality CAMs are used as pseudo-masks to supervise the segmentation result. Experimental results on the PASCAL VOC 2012 dataset demonstrate that our method significantly outperforms other state-of-the-art methods, achieving 67.2% and 68.76% mIoU on PASCAL VOC 2012 val set and test set, respectively. Furthermore, our method has been extended to weakly supervised object localization task, and experimental results demonstrate that our method continues to achieve very competitive results.

==> figs_tables/table4_old.tex <==
\begin{table*}[tb]
\begin{center}
%\renewcommand\arraystretch{1.6}
%\setlength{\tabcolsep}{10pt}{
\caption{Comparsion of MaxBoxAccV2 scores and localization performance on the CUB-200-2011 based on VGG16 and ResNet50 using different methods.}
\begin{tabular}{l|cccc|ccc|cccc|ccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{7}{c|}{VGG16} & \multicolumn{7}{c}{ResNet50} \\ \cline{2-15} 
 & \multicolumn{3}{c}{$\delta$} & \multicolumn{1}{l|}{\multirow{2}{*}{Mean}} & \multicolumn{1}{c}{\multirow{2}{*}{loc-1}} & \multirow{2}{*}{loc-5} & \multirow{2}{*}{GT Loc} & \multicolumn{3}{c}{$\delta$} & \multicolumn{1}{c|}{\multirow{2}{*}{Mean}} & \multirow{2}{*}{loc-1} & \multirow{2}{*}{loc-5} & \multirow{2}{*}{GT Loc} \\
 & 0.3 & 0.5 & 0.7 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{} &  &  & 0.3 & 0.5 & 0.7 & \multicolumn{1}{c|}{} &  &  &  \\ \hline
CutMix~\cite{yun2019cutmix} & 91.10 & 67.30 & 28.60 & \multicolumn{1}{l|}{62.30} & - & - & - & 94.30 & 71.50 & 22.50 & \multicolumn{1}{l|}{62.80} & 54.81 & - & - \\
Ki et al~\cite{ki2020sample} & 96.20 & 77.20 & 26.80 & \multicolumn{1}{l|}{66.70} & 57.50 & - & - & 96.20 & 72.80 & 20.60 & \multicolumn{1}{l|}{63.20} & 56.10 & - & - \\

%CALM & - & - & - & \multicolumn{1}{l|}{64.8} & - & - & - & - & - & - & \multicolumn{1}{l|}{71.0} & - & - & - \\
CREAM~\cite{xu2022cream} & - & - & - & \multicolumn{1}{l|}{62.20} & 70.44 & 85.67 & 90.98 & - & - & - & \multicolumn{1}{l|}{64.90} & \textbf{76.03} & - & 89.88\\
%BAS~\cite{wu2022background} & - & - & - & \multicolumn{1}{l|}{-} & 71.33 & 85.33 & 91.07 & - & - & - & \multicolumn{1}{l|}{-} & 77.25 & 90.08 & 95.13\\
BagsCAM~\cite{zhu2022bagging} & - & - & - & \multicolumn{1}{l|}{-} & -  & - & - & - & - & - & \multicolumn{1}{l|}{\textbf{84.88}} & 69.67  & -  &  \textbf{94.01}\\
KD-CI-CAM~\cite{shao2023further} & - & - & - & \multicolumn{1}{l|}{-} & \textbf{73.00} & 86.50 & 91.60 & - & - & - & \multicolumn{1}{l|}{-} & -  & -  & -\\
Bridging~\cite{kim2022bridging} & 99.30 & 93.20 & 47.80 & \multicolumn{1}{l|}{80.10} & 70.83 & 88.07 & 93.17 & 99.40 & 90.40 & 38.00 & \multicolumn{1}{l|}{75.90} & 73.16 & 86.68 & 91.60 \\

Bridging+Ours & \textbf{99.36} & \textbf{93.84} & \textbf{57.00}  & \multicolumn{1}{l|}{\textbf{84.31}} & 70.76  & \textbf{88.25} & \textbf{93.91} &  \textbf{99.40} &  \textbf{92.20} &\textbf{54.00} & \multicolumn{1}{l|}{81.90} &  74.01 &  \textbf{87.87} & 92.32
\end{tabular}\label{tab4}
\end{center}
\end{table*}

==> figs_tables/table5_coco.tex <==
\begin{table}[t]
\begin{center}
\renewcommand\arraystretch{1.6}
\setlength{\tabcolsep}{10pt}{
\caption{Comparisons to the state-of-the-art methods on the \emph{val} sets of MS COCO 2014~\cite{lin2014microsoft} in terms of mIoU ($\%$). ``Superv.'' is the corresponding training supervision ($\mathcal{I}$: image-level class label, $\mathcal{S}$: saliency masks).}
\begin{tabular}{ l c c | c } 
Methods & Backbone & Superv.  & \emph{val} (\%)\\ 
\hline \hline
\multicolumn{4}{l}{(\textbf{a}) \textbf{\emph{Large Vision Models}}} \\ 
\cdashline{1-4}[0.8pt/2pt]
SAM~\cite{kirillov2023segany,sun2023alternative} & ResNet-101 & $\mathcal{I}$ & 55.6 \\
\hline \hline
\multicolumn{4}{l}{(\textbf{b}) \textbf{\emph{Multi-stage}}} \\ 
\cdashline{1-4}[0.8pt/2pt]
IAL~\cite{wang2020weakly} & VGG-16 & $\mathcal{I}$ & 27.70 \\
ADL~\cite{choe2020attention} & VGG-16 & $\mathcal{I}$  & 30.75 \\ 
IRN~\cite{ahn2019weakly} & ResNet-50 & $\mathcal{I}$ & 32.60 \\
SEAM~\cite{wang2020self} & WideResNet-38 & $\mathcal{I}$  &  31.90 \\
CONTA~\cite{zhang2020causal} & WideResNet-38 & $\mathcal{I}$  &  32.80 \\
RIB~\cite{lee2021reducing} & ResNet-101 & $\mathcal{I}$  &  43.80 \\
ReCAM~\cite{chen2022class} & ResNet-101 & $\mathcal{I}$  &  45.00 \\
MCTformer~\cite{xu2022multi}  & WideResNet-38 & $\mathcal{I}$  & 42.00  \\
\cdashline{1-4}[0.8pt/2pt]
\textbf{RTC} w/o CRF & WideResNet-38 & $\mathcal{I}$  & \textbf{--} \\
\textbf{RTC} & WideResNet-38 & $\mathcal{I}$  & \textbf{--} \\
\textbf{RTC} w/o CRF & MiT-B1 & $\mathcal{I}$  & \textbf{--} \\
\textbf{RTC} & MiT-B1 & $\mathcal{I}$  & \textbf{--} \\
\hline \hline
\multicolumn{4}{l}{(\textbf{c}) \textbf{\emph{Single-stage}}} \\ 
\cdashline{1-4}[0.8pt/2pt]
AFA~\cite{ru2022learning} & MiT-B1 & $\mathcal{I}$  & 38.90  \\
SLRNet~\cite{pan2022learning} & WideResNet-38 & $\mathcal{I}$  & 35.00  \\
TSCD~\cite{xu2023self} & MiT-B1 & $\mathcal{I}$  & 40.10  \\
ToCo~\cite{ru2023token} & MiT-B1 & $\mathcal{I}$  & 41.30  \\
\cdashline{1-4}[0.8pt/2pt]
\textbf{RTC} w/o CRF & WideResNet-38 & $\mathcal{I}$  &  \\ %\textbf{35.61}
\textbf{RTC} & WideResNet-38 & $\mathcal{I}$  &  \\ %\textbf{36.42}
\textbf{RTC} w/o CRF & MiT-B1 & $\mathcal{I}$  & \textbf{--} \\
\textbf{RTC} & MiT-B1 & $\mathcal{I}$  & \textbf{--} 
\end{tabular}
\label{tab5}}
\end{center}
\vspace{-2mm}
\end{table}

==> sections/6_bib.tex <==
%-----------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/wangchunyan.jpg}}]
{Chunyan Wang} is currently a Ph.D. student in School of Computer Science and Engineering, Nanjing University of Science and Technology, China. Before that, she received the BS degree and the MS degree in Computer Science and Technology at Nanjing Forestry University, China. Her research mainly focuses on deep learning, semantic segmentation and their applications. In these areas, she has published several journal papers including Neural Networks and Neurocomputing.
\end{IEEEbiography}
%-------------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/zhangdong.jpg}}]{Dong Zhang} received his Ph.D. degree in computer science and technology from Nanjing University of Science and Technology in 2021. Dr. Zhang is now a postdoctoral research scientist at the Department of Computer Science and Engineering, The Hong Kong University of Science and Technology. His research interests include machine learning, image processing, computer vision and medical image analysis, especially in image classification, semantic image segmentation, object detection, and their potential applications. In these areas, he has published several journal and conference papers including IEEE Trans Cybern, PR, AAAI, ACM MM, IJCAI, ECCV, ICCV, and NeurIPS.
\end{IEEEbiography}
%-------------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/liyanzhang.jpg}}]
{Liyan Zhang} received the Ph.D. degree in computer science from the University of California, Irvine, Irvine, CA, USA, in 2014. She is currently a Professor with the College of Computer Science and Technology, Nanjing University of Aeronautics and Astronautics, Nanjing, China. Her research interests include multimedia analysis, computer vision, and deep learning. Dr. Zhang received the Best Paper Award from the International Conference on Multimedia Retrieval (ICMR) 2013 and the Best Student Paper Award from the International Conference on Multimedia Modeling (MMM) 2016.
\end{IEEEbiography}
%-------------------------------------------------------------------------
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/jinhuitang.jpg}}]
{Jinhui Tang} (Senior Member, IEEE) received the B.E. and Ph.D. degrees from the University of Science and Technology of China, Hefei, China, in 2003 and 2008, respectively. He is currently a Professor with the Nanjing University of Science and Technology, Nanjing, China. He has authored more than 150 articles in top-tier journals and conferences. His research interests include multimedia analysis and computer vision. Dr. Tang was a recipient of the Best Paper Awards in ACM MM 2007, PCM 2011, ICIMCS 2011, and ACM MM Asia 2020, the Best Paper Runner-Up in ACM MM 2015, and the Best Student Paper Awards in MMM 2016 and ICIMCS 2017. He has served as an Associate Editor for the IEEE TNNLS, the IEEE TKDE, and the IEEE TMM.
\end{IEEEbiography}
%-------------------------------------------------------------------------
